Learning in Feedback-driven Recurrent Spiking Neural Networks using full-FORCE Training

Feedback-driven recurrent spiking neural networks (RSNNs) are powerful computational models that can mimic dynamical systems. However, the presence of a feedback loop from the readout to the recurrent layer de-stabilizes the learning mechanism and prevents it from converging. Here, we propose a supervised training procedure for RSNNs, where a second network is introduced only during the training, to provide hint for the target dynamics. The proposed training procedure consists of generating targets for both recurrent and readout layers (i.e., for a full RSNN system). It uses the recursive least square-based First-Order and Reduced Control Error (FORCE) algorithm to fit the activity of each layer to its target. The proposed full-FORCE training procedure reduces the amount of modifications needed to keep the error between the output and target close to zero. These modifications control the feedback loop, which causes the training to converge. We demonstrate the improved performance and noise robustness of the proposed full-FORCE training procedure to model 8 dynamical systems using RSNNs with leaky integrate and fire (LIF) neurons and rate coding. For energy-efficient hardware implementation, an alternative time-to-first-spike (TTFS) coding is implemented for the full- FORCE training procedure. Compared to rate coding, full-FORCE with TTFS coding generates fewer spikes and facilitates faster convergence to the target dynamics.

==> sections/methods.tex <==
\subsection{FORCE Algorithm}





\subsection{Full-FORCE Algorithm}
The full-FORCE algorithm incorporates two networks, a target generating network that is used during training and a task performing network. The activity of the N-unit network is given by :


\begin{figure}[h!]
    \centering
	%\begin{center}
	    %\vspace{-40pt}
		\includegraphics[width=0.99\columnwidth]{sections/images/eqn1.png}
		%\vspace{-20pt}
	%\end{center}
	%\caption{Variation of the two features for 1.2 seconds.}% related to this proposal.}
	\label{fig:features}
\end{figure}

where τ is the time scale of the network dynamics, H is a nonlinear function that maps the vector of network activities xD into a corresponding vector of “firing rates” H(x)= tanh(x).  An input fin(t) is provided to the network units through a vector of input weights uin. The output of the network, z(t), is defined as a sum of unit firing rates weighted by a vector w,
\begin{figure}[h!]
    \centering
	%\begin{center}
	    %\vspace{-40pt}
		\includegraphics[width=0.99\columnwidth]{sections/images/output eqn.png}
		%\vspace{-20pt}
	%\end{center}
	%\caption{Variation of the two features for 1.2 seconds.}% related to this proposal.}
	\label{fig:features}
\end{figure}

The connection matrix JD is an N × N matrix of recurrent connections between network units randomly initiated with elements from a Gaussian distribution with zero mean and variance g2/N. The g value is slightly greater than 1 (for all of the examples we present here, g = 1.5), meaning that, in the absence of any input, the target-generating network would exhibit chaotic activity [16]. However, importantly, this chaotic activity is suppressed by the two inputs included in Eq 7. The new input term, not present in Eq 1, delivers the target output fout(t) into the network through a vector of weights u. The components of u, like those of uin, are chosen i.i.d. from a uniform distribution between -1 and 1.
\subsection{Leaky-Integrate-and-Fire Networks}


\subsection{Encoding Techniques}


\subsection{Experiments}
